Recy-ctronics: Designing Fully Recyclable Electronics With Varied Form Factors

For today's electronics manufacturing process, the emphasis on stable functionality, durability, and fixed physical forms is designed to ensure long-term usability. However, this focus on robustness and permanence complicates the disassembly and recycling processes, leading to significant environmental repercussions. In this paper, we present three approaches that leverage easily recyclable materials-specifically, polyvinyl alcohol (PVA) and liquid metal (LM)-alongside accessible manufacturing techniques to produce electronic components and systems with versatile form factors. Our work centers on the development of recyclable electronics through three methods: 1) creating sheet electronics by screen printing LM traces on PVA substrates; 2) developing foam-based electronics by immersing mechanically stirred PVA foam into an LM solution; and 3) fabricating recyclable electronic tubes by injecting LM into mold cast PVA tubes, which can then be woven into various structures. To further assess the sustainability of our proposed methods, we conducted a life cycle assessment (LCA) to evaluate the environmental impact of our recyclable electronics in comparison to their conventional counterparts.

==> contents/02_related_work.tex <==
\section{Related Work}
\subsection{Printed Electronics}
Printed electronics represents a cutting-edge technology that involves fabricating electronic devices and circuits through various printing methods, such as inkjet printing \cite{nayak2019review}, screen printing \cite{cheng2023swellsense} and 3D printing \cite{wang2018printed,valentine2017hybrid}. These printing techniques can also be combined with different pre/post-treatments for versatile use cases. For instance, conformally transfer printed heat-shrinkage film-based electronics can be applied to complex 3D surfaces \cite{rich2022developing}. Creating pre-strain or cutting patterns can enable stretchable electronics \cite{kim2008materials, talyan2023kirisense}. Printed electronics offer several advantages, including the creation of lightweight, mostly flexible or stretchable electronic components, circuits, or even systems. The manufacturing approach can also be more sustainable by favoring more on additive over subtractive methods.

Within the Human-Computer Interaction (HCI) community, rapid prototyping is a key theme for printed electronics research. One pioneering example is \textit{Instant Inkjet Circuits}, which introduced the use of commodity inkjet printers for quickly prototyping functional devices \cite{kawahara2013instant}. Building on this accessible and diverse design concept, researchers have utilized this technique to fabricate various sensors \cite{cheng2020silver, pourjafarian2019multi, yan2022fibercuit}, antennas \cite{li2016paperid}, displays \cite{olberding2014printscreen} and even heating-based actuators \cite{olberding2015foldio}. Moreover, researchers have demonstrated the scalability of printed electronics beyond the normal machine sizes. For example, \textit{Sprayable} introduced a spraying technique for prototyping large-scale sensors and displays \cite{wessely2020sprayable}, while \textit{Duco} introduced a system that leverages a hanging wall robot to draw large-scale circuits directly on everyday surfaces, using multiple tools and substrates.

\subsection{Recyclable Electronics}
With the remarkable advancements in fabricating diverse electronics, spanning various form factors, scales, and functionalities, the issue of disposing of these devices has become a pressing concern, yet not much effort has been devoted to this problem within the HCI community. Song et al. proposed a method to manufacture wireless heating interfaces that can decompose in backyard conditions within 60 days \cite{song2022towards}. \textit{Functional Destruction} is another recent work demonstrated three different approaches (PVA, beeswax and edible chocolate) to make electronics that are physically and functionally transient \cite{cheng2023functional}. Lazaro Vasquez et al. focused on mycelium, which is a fast-growing vegetative part of a fungus, to replace the plastic housing for traditional PCBs, but most of these work aims to make electronics with disposable or degradable manners instead of recyclable \cite{lazaro2019plastic}. The only two works, which are both from the same research group, try to emphasize recyclability for electronics. Arroyos et al. introduced an end-to-end digital fabrication process for creating a computer mouse with a biodegradable printed circuit board and case, utilizing materials like Jiva Soluboard and PVA 3D printing filament \cite{arroyos2022tale}, where the electronic components can be reused in this case. The other work expands the recyclability from the components to the substrate and the electrode material. Zhang et al. present vPCB, using vitrimer as the replacement for conventional circuit boards with a high recycling rate \cite{zhang_recyclable_2024}.

In contrast, other research fields such as materials science and electrical engineering have delved extensively into recycling electronics. Khrustalev et al., for instance, deviated from conventional thermoset materials like fiberglass and epoxy and instead used thermoplastic materials (3D printing PLA) as the substrate, showcasing how electronics can be fabricated and recycled efficiently \cite{khrustalev2022new}. \textit{3R} project also aims to design resilient, repairable, and recyclable electronics through a combination of novel biphasic printable LM composites and reversible tough block co-polymers \cite{tavakoli20223r}. LM, known for its excellent conductivity and intrinsic fluid nature, has been widely used as an electrode option for recyclable electronics. Teng et al. demonstrated two papers utilizing LM as the conductive material and PVA and beeswax as the substrate materials, respectively \cite{teng2019liquid, teng2023fully}. The beeswax approach stands out as it features a self-destructing-recycling process where the LM traces react with the sodium hydroxide within the device. These projects share a common goal of adapting straightforward recycling approaches that avoid complicated procedures or tooling while achieving high recyclability rates.

\subsection{Sustainable Computing}
The proliferation of miniaturized computational devices has brought up a range of environmental hazards, from plastic waste, E-waste to unsustainable power consumption. The call for sustainability echoes across industries, urging designers, researchers and makers to adopt more environmentally conscious materials and practices~\cite{mankoff2007environmental, lazaro2020introducing, brynjarsdottir2012sustainably, disalvo2010mapping, blevis2007sustainable, zhang_biodegradable_2024}. For material selection, even when eco-friendly options like PLA hold promise, it is always challenging to source from responsible manufacturers and find proper disposal avenues. Another critical area drawing from the use of traditional batteries~\cite{hester2017future,lucia2017intermittent}. While harvesting energy from various sources shows potential, it alone cannot ensure continuous device operation, prompting the need for solutions like energy buffering with capacitors to enable intermittent computing~\cite{de2020battery,bakar2022protean}. In the pursuit of sustainable alternatives, batteryless energy-harvesting devices have emerged as promising contenders, challenging the dominance of battery-powered counterparts with their eco-friendliness and reduced maintenance requirements~\cite{ferrese2015battery,de2022dips,bakar2021rehash, iyer_wind_2022}. Lastly, the concept of Life Cycle Assessment (LCA) is a cradle-to-grave method to study a device's environmental impact, which has guided researchers to evaluate whether a device is more or less sustainable in a more quantitative manner ~\cite{lazaro2020introducing}. 




\begin{figure*}[h]
  \centering
  \includegraphics[width=1\linewidth]{Figures/sheet_testing.png}
  \caption{General design strategy. (a) Load versus strain curve under uniaxial deformation for different types of PVA and Cyclic loading to increasing strains as a function of strain. (b) Demonstration of PVA's mechanical flexibility (rigid, highly flexible, stretchable) for versatile types of devices (sheet, foam, tube). 
 }~\label{figure:testing1}
\end{figure*}


==> contents/07_recycle_process.tex <==
\section{Recycling Process}
We have introduced Recy-ctronics for crafting interactive devices across varying form factors. These devices not only offer diverse interaction capabilities but are also designed with full recyclability in mind. The recycling process is the same for all three form factors—sheet, foam, and tube, while recycling rates, duration, and practical viability might differ among different form factors.

The recycling process follows prior literatures \cite{teng2019liquid, xu2021printable, teng2023fully}, which starts with detaching electronic components if there are any (\textit{e.g.,} SMD, MCU, battery) from the substrates. Any material remnants on the pins of the components can be delicately eliminated using tweezers or by partially immersing them in water. Any components can be further dried out to prevent electrical failure under the condition of 80-90°C for one day in a laboratory oven. Then the entire device undergoes immersion in water until complete dissolution is achieved. Throughout this process, the dissolved device is subjected to thorough rinsing with fresh water, a step conducted 2-3 times to ensure the complete dissolution of PVA. The resulting PVA-enriched water is then collected, following the separation of the PVA-rich water from the residual LM fraction, approximately 5ml solution of 1mol\% NaOH is added to the LM. The quantity of NaOH solution is contingent upon the device's size. This NaOH serves the role of removing the oxidized layer on the LM, a thin Ga${2}$O${3}$ shell, thereby enabling the seamless recycling of the LM and ensuring high recycling efficiency. With the removal of the oxidized layer and the transformation of the LM into a spherical form, one can retrieve the LM by using a syringe. 

To assess the recycling performance across three distinct form factors, we carried out comprehensive recycling testing. This encompassed recycling an LED pattern on a thin sheet, a cylindrical conductive foam, and a 4cm pipe. The recycling process was executed with six samples for each design, documenting and presenting the pre- and post-recycling weights of PVA and LM. As shown \textcolor{blue}{Figure \ref{figure:recycletest}}, all three sample groups achieved a high recycling rate over 95\% on average for LM, where we have achieved 97.5\%, 96.1\% and 98.6\% for sheet, foam and tube respectively. Also the loss of PVA during the recycling process is higher, where we obtained 87.4\%, 78.1\% and 83.2\% for sheet, foam and tube respectively. Among all the three types of interactive devices, the tube group displayed the highest recycling rate for LM. This lower recycling rate for LM can potentially come from the foam's highly porosity structure, which is mostly covered by LM, inducing more oxidized area compared to sheets and tubes. 



Beyond the individual device recycling test phase, we expanded our scope to include a batch of devices accumulated over two months, leading to the recovery of 17.4 grams of LM, as detailed in \textcolor{blue}{Figure \ref{figure:recycletest}} b. This batch consisted of various device types (\textit{e.g.,} sheets, foams, tubes) and miscellaneous non-device waste, totaling 716 grams. Within approximately 30 hours, all materials dissolved in water, which is later rinsed three times to transport the PVA-rich water from the LM remnants. It is worth noting that we paid more attention to recycling LM for this experiment and saved the PVA solutions in containers for later prototyping use.

This lab-scale recycling initiative revealed several insights: (1) \textbf{Complexity in Bulk Processing}: Recycling a multitude of devices introduces complexities that we did not encounter in single-device recycling. The diverse mixture resulted in the emergence of unexpected contaminants such as silver epoxy particles, paper scraps, and wires, requiring further filtration through a 200 mesh filter (around 75 microns). (2) \textbf{Necessity for Improved Sorting}: The heterogeneous nature of the waste highlighted the need for a better sorting system. Varied material compositions with different ratios of glycerin, PVA, and de-ionized water, suggest pre-recycling categorization could stabilize the material composition of recycled outputs. (3) \textbf{Observations on LM Recycling}: The bulk recycling process yielded a higher presence of oxidized substances and an increase in the resistance of the recycled LM, with a sheet resistance of 0.019$\pm$0.011 $\Omega/sq$ (20 pieces of 40cm by 0.5cm samples), compared to the original LM's 0.013$\pm$0.002 $\Omega/sq$, which might stem from the extended environmental exposure during waste accumulation. (4) \textbf{Challenges in Dissolving PVA}: We have observed that the dissolving process dramatically slowed down after several hours, and we had to add more water to the dissolving tank. Also, approaching the end of the dissolving stage, we picked up some remained PVA fragments and separately dissolved them in a beaker with hot water. Overall, this experience with recycling accumulated waste underlines the method's simplicity and efficiency, making it particularly suitable for maker environments.

\begin{figure*}[h]
  \centering
  \includegraphics[width=1\linewidth]{Figures/recycle.png}
  \caption{Recycling process. (a) All three form factors-sheet, foam and tube will undergo immersion in the water until complete dissolution. Then the LM and PVA will be separately collected to conclude the recycling process. (b) Lab-scale recycling experiment over two months. 
 }~\label{figure:recycletest}
\end{figure*}
